Extending the Continuum of Six-Colorings

We present two novel six-colorings of the Euclidean plane that avoid monochromatic pairs of points at unit distance in five colors and monochromatic pairs at another specified distance $d$ in the sixth color. Such colorings have previously been known to exist for $0.41 < \sqrt{2} - 1 \le d \le 1 / \sqrt{5} < 0.45$. Our results significantly expand that range to $0.354 \le d \le 0.657$, the first improvement in 30 years. Notably, the constructions underlying this were derived by formalizing colorings suggested by a custom machine learning approach.

==> figures/firstcoloring/animation.tex <==
\tikzset{every picture/.style={scale=2}}

\newcommand{\centertriangle}[1]{%
    \coordinate (A) at ([shift=(270:\tc)](0,0);
    \coordinate (B) at ([shift=(150:\tc)](0,0);
    \coordinate (C) at ([shift=(30:\tc)](0,0);
    
    \draw[fill=#1] (A) -- (B) -- (C) -- cycle; 
    
    % \draw (A) -- ++(60:0.1) arc (60:120:0.1) -- cycle;
}


\newcommand{\blob}[4]{%
    \begin{scope}[rotate around={#3:(0,0)}]]
    \begin{scope}[shift={(#1,#2)}]
        \coordinate (A) at (0,0);
        
        \coordinate (B) at ([shift=(150:\tc)]A);
        \coordinate (C) at ([shift=(30:\tc)]A);
        
        \coordinate (BB) at ([shift=(150:\bd)]A);
        \coordinate (CC) at ([shift=(30:\bd)]A);
        
        \coordinate (BBB) at ([shift=(150-\pat/2:\pst)]BB);
        \coordinate (CCC) at ([shift=(30+\pat/2:\pst)]CC);

        \coordinate (E) at ([shift=(\bait:1)]B);
        \coordinate (D) at ([shift=(180-\bait:1)]C);
        
        \draw[fill=#4] (E) -- (CCC) -- (CC) -- (C) -- (B) -- (BB) -- (BBB) -- (D) -- cycle;


        % \draw[thick, color=purple] (D) -- ++(0,\ph+\bst+\th);
        % \draw[thin, color=green] (D) -- ++(0,1);
        
        % \draw[ultra thin, color=purple] (A) -- ++(30:0.3) arc (30:150:0.3) -- cycle;
        % \draw[ultra thin, color=purple] (BB) -- ++(-30:0.11) arc (-30:-30+\batm:0.11) -- cycle;
        % \draw[ultra thin, color=purple] (CC) -- ++(180:0.12) arc (180:180-\batrapt:0.12) -- cycle;
        % \draw[ultra thin, color=purple] (BBB) -- ++(0:0.11) arc (0:0-\batrapb:0.11) -- cycle;
        % \draw[ultra thin, color=purple] (BBB) -- ++(0:0.12) arc (0:0+\bamx:0.12) -- cycle;
        % \draw[ultra thin, color=purple] (BBB) -- ++(\bamx:0.12) arc (\bamx:\bamx+\faf:0.12) -- cycle;
        % \draw[ultra thin, color=purple] (D) -- ++(0:0.11) arc (0:0-\bait:0.11) -- cycle;
        % \draw[ultra thin, color=purple] (D) -- ++(\pab:0.12) arc (\pab:\pab+\fas:0.12) -- cycle;
        
        % \draw[ultra thin, color=blue] (BB) + (0.2,0) -- ++(0.2,\bhm);
        % \draw[ultra thin, color=blue] (D) -- ++(0,-\bhb);
        % \draw[ultra thin, color=blue] (B) + (\tl/2,0) -- ++(\tl/2,\bh);
        % \draw[ultra thin, color=blue] (BB) - ++(\bwt,0);
        % \draw[ultra thin, color=blue] (BBB) - ++(\bwb,0);
        
        % \draw[thin] (D) -- (C);
        % \draw[thin] (E) -- (B);
        
        % \draw[thin] (BB) -- (CCC);
        % \draw[thin] (BBB) -- (CC);
        
    \end{scope}
    \end{scope}
}


\newcommand{\flup}[4]{%
    \begin{scope}[rotate around={#3:(0,0)}]]
    \begin{scope}[shift={(#1,#2)}]

        \coordinate (A) at (0,0);
        \coordinate (B) at ([shift=(180-\pab:\pss)]A);
        \coordinate (C) at ([shift=(-\pab+\faf:\bsb)]B);
        \coordinate (D) at ([shift=(-\pab+\faf-180+\fas:\pss)]C);
        \coordinate (E) at ([shift=(-\pab+2*\faf+\fas:\bsb)]D);
        \coordinate (F) at ([shift=(-\pab+2*\faf+2*\fas-180:\pss)]E);
        
        \draw[fill=#4]  (A) -- (B) -- (C) -- (D) -- (E) -- (F) --cycle;

            
        % \draw (A) -- ([shift=(180-\pab-\fad:\fd)]A);
        % \draw[ultra thin, color=blue] (A) -- ++(180-\pab:0.1) arc (180-\pab:180-\pab-\fad:0.1) -- cycle;
        
        % \draw[ultra thin, color=blue] (A) -- ++(180-\pab:0.11) arc (180-\pab:180-\pab-\fas:0.11) -- cycle;
                
        % \draw[ultra thin, color=blue] (B) -- ++(-\pab:0.1) arc (-\pab:-\pab+\faf:0.1) -- cycle;
        
        % \draw[ultra thin, color=blue] (C) -- ++(360-\pab-\fad:0.1) arc (360-\pab-\fad:360-\pab-\fad-\fadd:0.1) -- cycle;
        
        % \draw[ultra thin, color=blue] (C) -- ++(360-\pab-\fad:0.11) arc (360-\pab-\fad:360-\pab-\fad+\faddd:0.11) -- cycle;

        % \draw[dotted] (A) circle (\fw);
    \end{scope}
    \end{scope}
}


\newcommand{\pentagon}[4]{%
    \begin{scope}[rotate around={#3:(0,0)}]]
    \begin{scope}[shift={(#1,#2)}]

        \coordinate (A) at (0,0);
        \coordinate (B) at ([shift=(90-\pat/2:\pst)]A);
        \coordinate (C) at ([shift=(90+\pat/2:\pst)]A);
        
        \coordinate (D) at ([shift=(90-\pait/2:\avoid)]A);
        \coordinate (E) at ([shift=(90+\pait/2:\avoid)]A);
    
        \draw[fill=#4] (A) -- (B) -- (D) -- (E) -- (C) -- cycle;


        % \draw[thick, color=purple] (A) -- ++(0,-\bst-\th);
        % \draw[ultra thin, color=purple] (A) -- ++(0,\ph+\bhc-\bht);
        
        % \draw[ultra thin, color=blue] (B) -- ++(180:0.1) arc (180:180+\past:0.1) -- cycle;
        % \draw[ultra thin, color=blue] (C) -- ++(0:0.1) arc (0:0+\pasb:0.1) -- cycle;
        % \draw[ultra thin, color=blue] (A) -- ++(90-\pait/2:0.1) arc (90-\pait/2:90+\pait/2:0.1) -- cycle;
        % \draw[ultra thin, color=blue] (A) -- ++(90-\pat/2:0.1) arc (90-\pat/2:90+\pat/2:0.1) -- cycle;
        % \draw[ultra thin, color=blue] (D) -- ++(180:0.1) arc (180:180+\pab:0.1) -- cycle;
        
        % \draw[ultra thin, color=purple] (A) -- (B);
        % \draw[ultra thin, color=purple] (A) -- ++(0,\pht);
        % \draw[ultra thin, color=purple] (D) -- ++(0,-\phb);
        % \draw[ultra thin, color=purple] (E) -- ++(0,-\pss);
        % \draw[ultra thin, color=purple] (D) -- ++(-\psb,0);
        
        % \draw[thin] (D) -- (A) -- (E);
        % \draw[thin] (B) -- (C);
    \end{scope}
    \end{scope}
}

\newcommand{\block}[2]{%
    \begin{scope}[shift={(#1,#2)}]
    
    \flup{\psb/2}{\bhc}{0}{lturquoise}
    \draw[thick] (B) -- (C) -- (D) -- (E);
    
    \begin{scope}[xscale=-1]
        \flup{+\psb/2}{\bhc}{0}{lyellow}
        \draw[thick] (B) -- (C) -- (D) -- (E);
    \end{scope}

    
    \blob{0}{0}{0}{lgreen}
    \blob{0}{0}{-120}{lblue}
    \draw[thick]  (BBB) -- (D) -- (E) -- (CCC) -- (CC);
    \blob{0}{0}{120}{lorange}
    \draw[thick]  (BB) -- (BBB) -- (D) -- (E) -- (CCC);

    \pentagon{0}{-\bhc-\ph}{180}{lred}
    \draw[thick] (C) -- (A) -- (B);
    % \pentagon{0}{-\bhc-\ph}{60}{lred}
    % \pentagon{0}{-\bhc-\ph}{-60}{lred}
    
    % \pentagon{0}{\bd}{180}{lred}
    \pentagon{0}{\bd}{-60}{lred}
    \draw[thick] (B) -- (D) -- (E);
    \pentagon{0}{\bd}{60}{lred}
    \draw[thick] (D) -- (E) -- (C);
    
    \centertriangle{lred}
        
    \end{scope}
}

\newcommand{\coloring}{
    \clip (-4,-1.7) rectangle (+4,+2.5);
    
    \begin{scope}[shift={(-2*\sx,0)}, opacity=0.3]
    \block{0}{2*\height}
    \block{0}{\height}
    \block{0}{0}
    \block{0}{-\height}
    \block{0}{-2*\height}
    \end{scope}
    
    \begin{scope}[shift={(-\sx, \height-\sy)}, opacity=0.3]
        \block{0}{\height}
        \block{0}{0}
        \block{0}{-\height}
        \block{0}{-2*\height}
    \end{scope}
    
    \begin{scope}[opacity=0.3]
    \block{0}{2*\height}
    \block{0}{\height}
    \block{0}{-\height}
    \block{0}{-2*\height}
    \end{scope}
    
    \block{0}{0}
    
    \begin{scope}[shift={(\sx, \sy)}, opacity=0.3]
        \block{0}{\height}
        \block{0}{0}
        \block{0}{-\height}
        \block{0}{-2*\height}
    \end{scope}
    
    \begin{scope}[shift={(2*\sx,0)}, opacity=0.3]
    \block{0}{2*\height}
    \block{0}{\height}
    \block{0}{0}
    \block{0}{-\height}
    \block{0}{-2*\height}
    \end{scope}
    
    \circles{(0,\bhc+\ph)}
    
    \begin{scope}[rotate around={60:(0,0)}]]
    \circles{(\psb/2,-\bhc)}
    \end{scope}
    
    \begin{scope}[rotate around={60:(0,0)}]]
    \circles{(-\avoid/2,\bd+\pht)}
    \end{scope}
}

\begin{animateinline}[autoplay,loop]{6}
    \multiframe{20}{rAvoid=0.354+0.01}{
        \begin{tikzpicture}
        \pgfmathsetmacro{\avoid}{\rAvoid}
        \input{figures/firstcoloring/variables}  
        \coloring
        \end{tikzpicture}
    }
\end{animateinline}


==> figures/firstcoloring/variables.tex <==
% Pentagon variables
\pgfmathsetmacro{\pat}{(\avoid-0.354)*70.9 + 113.7 }               % Wide angle at top
\pgfmathsetmacro{\pst}{(\avoid / 2) * cosec(\pat / 2)}             % Side length at top
\pgfmathsetmacro{\pait}{2*acos(cosec(\pat / 2)/4)) - \pat}         % Inner acute angle at top
\pgfmathsetmacro{\psb}{2 * \avoid * sin(\pait/2)}                  % Side length at bottom
\pgfmathsetmacro{\ph}{cos(\pait/2) * \avoid}                       % Total height of pentagon
\pgfmathsetmacro{\pht}{ cos(\pat/2)*\pst}                          % Height of top triangle
\pgfmathsetmacro{\phb}{\ph - \pht}                                 
\pgfmathsetmacro{\pss}{sqrt(\phb^2+(\avoid-\psb)^2/4 )}            % Side length at side
\pgfmathsetmacro{\past}{90-\pat/2}                                 % Angle at side top part
\pgfmathsetmacro{\pasb}{asin(\phb/\pss)}                           % Angle at side bottom part
\pgfmathsetmacro{\pas}{\past+\pasb}                                % Angle at side
\pgfmathsetmacro{\pab}{270-\pat/2-\pas}                            % Angle at bottom


% Triangle variables
\pgfmathsetmacro{\bd}{((sqrt(1 - (\pst * sin(30+\pat/2))^2) - \pst * cos(30+\pat/2)))/sqrt(3)}
\pgfmathsetmacro{\tc}{max(\bd-\avoid,0)}                   % Max distance of triangle from center
\pgfmathsetmacro{\tl}{sqrt(3)*\tc}                         % Length of side of triangle
\pgfmathsetmacro{\th}{3/2*\tc}                             % Height of triangle


% Octagon variables
\pgfmathsetmacro{\bwt}{2*sin(60)*\bd}                                      % Blob upper width
\pgfmathsetmacro{\batrapb}{180-acos((1-\bwt^2-\pst^2)/(-2*\bwt*\pst))}     % Angle of trapezoid bottom
\pgfmathsetmacro{\bwb}{\pst*cos(\batrapb)+sqrt(1-\pst^2*sin(\batrapb)^2)}  % Blob lower width
\pgfmathsetmacro{\bait}{acos((\tl+\psb)/2)}                                %
\pgfmathsetmacro{\bh}{cos(90-\bait)}                                       % Total height of blob
\pgfmathsetmacro{\bhc}{\bh + \th - \tc}                                    % Total height of blob from center
\pgfmathsetmacro{\bhtc}{sqrt(\bd^2-(\bwt/2)^2)}                            % Height of top from center
\pgfmathsetmacro{\bht}{\bhtc - (\th - \tc)}                                % Height of top
\pgfmathsetmacro{\bhm}{sqrt(\pst^2-(abs(\bwt-\bwb)/2)^2)}                  % Height of trapezoid
\pgfmathsetmacro{\bhb}{\bh - \bht - \bhm}                                  % Height of bottom
\pgfmathsetmacro{\bsb}{sqrt(\bhb^2 + (\bwb/2-\psb/2)^2)}                   % Side at bottom not adjacent to pentagon
\pgfmathsetmacro{\bat}{150}
\pgfmathsetmacro{\bast}{180-\pat/2}
\pgfmathsetmacro{\basb}{atan(\bhb / (\bwb/2-\psb/2))+\batrapb}
\pgfmathsetmacro{\bab}{540-\bat-\basb-\bast}



% Hexagon variables
\pgfmathsetmacro{\faf}{360 - \basb - \pas}    
\pgfmathsetmacro{\fas}{240 - \faf} 

\pgfmathsetmacro{\fd}{sqrt(\pss^2 + \bsb^2 - 2*\pss*\bsb*cos(\faf))}
\pgfmathsetmacro{\fad}{asin(\bsb*sin(\faf)/\fd)}
\pgfmathsetmacro{\fadd}{(180-\faf-\fad)}
\pgfmathsetmacro{\faddd}{(\fas-\fadd)}
\pgfmathsetmacro{\fw}{sqrt(\fd^2+\pss^2-2*\fd*\pss*cos(\faddd))}

% Other variables
\pgfmathsetmacro{\height}{\ph+\bhc+\bd}  % Total height of construction
\pgfmathsetmacro{\ts}{\bhc+\bd+\ph}
\pgfmathsetmacro{\sx}{\ts*cos(30)}
\pgfmathsetmacro{\sy}{\ts*sin(30)}

% asserts
\newcommand{\assert}[2]{%
    \pgfmathparse{#1}%
    \let\resultA=\pgfmathresult%
    \pgfmathparse{#2}%
    \let\resultB=\pgfmathresult%
    \ifdim\resultA pt>\resultB pt\relax%
        \errmessage{Assertion failed for condition: #1 <= #2}%
    \fi
}

\assert{\tl}{\avoid}
\assert{\avoid}{\bsb}
\assert{\bwb}{1}
\assert{\bwt}{1}
\assert{\fw}{1}
\assert{1}{\avoid+\th+\ph}


% Colors
\definecolor{lred}{HTML}{FFADAD}
\definecolor{lorange}{HTML}{FFD6A5}
\definecolor{lyellow}{HTML}{FDFFB6}
\definecolor{lgreen}{HTML}{CAFFBF}
\definecolor{lturquoise}{HTML}{9BF6FF}
\definecolor{lblue}{HTML}{A0C4FF}
\definecolor{lpurple}{HTML}{BDB2FF}
\definecolor{lpink}{HTML}{FFC6FF}

% Circles
\newcommand{\circles}[1]{%
    \begin{scope}[shift={(#1)}]
    
    \draw[fill=black] (0,0) circle (0.02);
    \draw[dashed, line width=0.1pt] (0,0) circle (\avoid);
    \draw[dotted, line width=0.4pt] (0,0) circle (1);
        
    \end{scope}
}

==> figures/secondcoloring/completelarge.tex <==

\pgfmathsetmacro{\scale}{1.5}
\tikzset{every picture/.style={scale=\scale}}

\input{figures/secondcoloring/variables}

\newcommand{\circles}[1]{%
    \begin{scope}[shift={(#1)}]
    
    \draw[fill=black] (0,0) circle (0.01);
    % \draw[dash dot, line width=0.1pt] (0,0) circle (\minavoid);
    % \draw[dashed, line width=0.1pt] (0,0) circle (\maxavoid);
    % \draw[dotted, line width=0.4pt] (0,0) circle (1);
    
    \draw[dotted, line width=0.4pt] (0,0) circle (1.6);
    
    \end{scope}
}

\newcommand{\block}[3]{%
    \begin{scope}[rotate around={#3:(0,0)}]]
    \begin{scope}[shift={(#1,#2)}]

        \coordinate (A) at (0, 0);
        \coordinate (AA) at (1, 0);
        \coordinate (MA) at (1/2, 0);
        \coordinate (PA) at (1/2, {sqrt(3)/2});
        
        \coordinate (C) at (1, {sqrt(3)});
        \coordinate (CC) at (2, {sqrt(3)});
        \coordinate (MC) at (3/2, {sqrt(3)});
        \coordinate (PC) at (3/2, {sqrt(3)/2});
        
        \coordinate (BB) at (-1, {sqrt(3)});
        \coordinate (B) at (0, {sqrt(3)});
        \coordinate (MB) at (-1/2, {sqrt(3)});
        \coordinate (PB) at (-1/2, {sqrt(3)/2});
        \coordinate (MAA) at (1/2, {- sqrt(3)/2 + \maxavoid});
        
        \coordinate (X) at (1/2, {sqrt(3)/2 - \maxavoid});
        \coordinate (Y) at (-1/2, {sqrt(3)/2 + \maxavoid});
        \coordinate (Z) at (3/2, {sqrt(3)/2 + \maxavoid});
        
        \coordinate (XXX) at ({1/2 + sqrt(3)/2 - \maxavoid}, 0);
        \coordinate (XX) at ({1/2 - sqrt(3)/2 + \maxavoid}, 0);
        \coordinate (YYY) at ({-1/2 - sqrt(3)/2 + \maxavoid}, {sqrt(3)});
        \coordinate (YY) at ({-1/2 + sqrt(3)/2 - \maxavoid}, {sqrt(3)});
        \coordinate (ZZZ) at ({3/2 + sqrt(3)/2 - \maxavoid}, {sqrt(3)});
        \coordinate (ZZ) at ({3/2 - sqrt(3)/2 + \maxavoid}, {sqrt(3)});

        \coordinate (U) at (1/4, {3*sqrt(3)/4 - \maxavoid/2});
        \coordinate (V) at (-1/4, {sqrt(3)/4 + \maxavoid/2});
        
        \coordinate (W) at (3/4, {3*sqrt(3)/4 - \maxavoid/2});
        \coordinate (R) at (5/4, {sqrt(3)/4 + \maxavoid/2});
    
        \coordinate (I2) at ([shift=(\auxa:\auxw)]V);
        \coordinate (I1) at ([shift=(\auxa:-\auxw)]U);

        \coordinate (I3) at ([shift=(180-\auxa:\auxw)]R);
        \coordinate (I4) at ([shift=(180-\auxa:-\auxw)]W);
 
        \coordinate (PD) at (1/2, {3/2*sqrt(3)});
        \coordinate (I5) at ($(PD) + (PA) - (I2)$);
        \coordinate (I6) at ($(PD) + (PA) - (I3)$);

        \coordinate (M) at (1/2-\auxx, {sqrt(3)-\auxy});
        \coordinate (N) at (1/2+\auxx, {sqrt(3)-\auxy});

        \coordinate (NN) at (1/2-\auxx, {sqrt(3)+\auxy});
        \coordinate (MM) at (1/2+\auxx, {sqrt(3)+\auxy});

        \pgfmathsetmacro{\yshift}{-sqrt(3)}
        \coordinate (MMM) at ([xshift=-1cm, yshift=\yshift cm)]MM);
        
        \pgfmathsetmacro{\yshift}{-sqrt(3)}
        \coordinate (NNN) at ([xshift=1cm, yshift=\yshift cm)]NN);
        
        \pgfmathsetmacro{\yshift}{-\scale*sqrt(3)}
        \begin{scope}[transform canvas={xshift = -\scale cm, yshift=\yshift cm}]
        \draw[fill=lorange] (Z) -- (ZZ) -- (C) -- (N) -- (I3) -- (I4) -- (PC) -- cycle;
        \end{scope}

        \begin{scope}[transform canvas={xshift = \scale cm, yshift=\yshift cm}]
        \draw[fill=lgreen] (Y) -- (YY) -- (B) -- (M) -- (I2) -- (I1) -- (PB) -- cycle;
        \end{scope}

        \begin{scope}[transform canvas={xshift=\scale cm, yshift = \yshift cm}]
        
        
        \draw[fill=lred] (PA) -- (I2) -- (M) -- (N) -- (I3)  -- cycle;
        \draw[fill=lblue] (M) -- (N) -- (C) -- (MM) -- (NN) -- (B) -- cycle;
        \draw[fill=lred] (I5) -- (MM) -- (NN) -- (I6) -- (PD) -- cycle;

        \end{scope}
        

        \draw[fill=lturquoise] (X) -- (XX) -- (A) -- (MMM) -- (I1) -- (I2) -- (PA) -- cycle;
        \draw[fill=lyellow] (X) -- (XXX) -- (AA) -- (NNN)  -- (I4) -- (I3) -- (PA) -- cycle;
        \draw[fill=lred] (X)-- (XX) -- (MAA)  -- (XXX) -- cycle;

        
    \end{scope}
    \end{scope}
}

\begin{tikzpicture}


\clip (-4,-3) rectangle (+6.6,+4);

    \begin{scope}[opacity=0.3]


    \block{-4.0}{2*sqrt(3)}{0}
    \block{-2.0}{2*sqrt(3)}{0}
    \block{0}{2*sqrt(3)}{0}
    \block{2.0}{2*sqrt(3)}{0}
    \block{4.0}{2*sqrt(3)}{0}
    \block{6.0}{2*sqrt(3)}{0}
    
    \block{7.0}{sqrt(3)}{0}
    \block{5.0}{sqrt(3)}{0}
    \block{3.0}{sqrt(3)}{0}
    \block{1.0}{sqrt(3)}{0}
    \block{-1.0}{sqrt(3)}{0}
    \block{-3.0}{sqrt(3)}{0}
    \block{-5.0}{sqrt(3)}{0}
    
    \block{6.0}{0}{0}
    \block{4.0}{0}{0}
    \block{2.0}{0}{0}
    \block{-2.0}{0}{0}
    \block{-4.0}{0}{0}
    
    \block{7.0}{-sqrt(3)}{0}
    \block{5.0}{-sqrt(3)}{0}
    \block{3.0}{-sqrt(3)}{0}
    \block{1.0}{-sqrt(3)}{0}
    \block{-1.0}{-sqrt(3)}{0}
    \block{-3.0}{-sqrt(3)}{0}
    \block{-5.0}{-sqrt(3)}{0}
    
    \block{6.0}{-2*sqrt(3)}{0}
    \block{4.0}{-2*sqrt(3)}{0}
    \block{2.0}{-2*sqrt(3)}{0}
    \block{0.0}{-2*sqrt(3)}{0}
    \block{-2.0}{-2*sqrt(3)}{0}
    \block{-4.0}{-2*sqrt(3)}{0}
    \end{scope}

    \block{0}{0}{0}

    % \circles{A}
    
    \begin{scope}[transform canvas={xshift = - 2*\scale cm}]
    \circles{X}
    \end{scope}

    
    \begin{scope}[transform canvas={xshift = 2*\scale cm}]
    \circles{PA}
    \end{scope}

    \pgfmathsetmacro{\yshift}{-\scale*sqrt(3)}
    \begin{scope}[transform canvas={xshift = 3*\scale cm, yshift = \yshift cm}]
    \circles{I1}
    \end{scope}
    
    \circles{N}
    
    \begin{scope}[transform canvas={xshift = 4*\scale cm}]
    \circles{XX}
    \end{scope}

    
    % \draw[very thin] (I1) circle[radius=0.5pt];

    

\end{tikzpicture}


==> figures/secondcoloring/variables.tex <==
% Distance variables
\pgfmathsetmacro{\maxavoid}{0.6570609747898615}
\pgfmathsetmacro{\minavoid}{sqrt(3) - 2*\maxavoid}

% Pentagon variables
\pgfmathsetmacro{\auxa}{atan(1/(2*\maxavoid+sqrt(3)))}
\pgfmathsetmacro{\auxl}{sqrt(1/4 + (sqrt(3)/2 + \maxavoid)^2)}
\pgfmathsetmacro{\auxw}{sqrt(3 - sqrt(3)*\maxavoid - \maxavoid^2)/2}

\pgfmathsetmacro{\auxx}{1/14}
\pgfmathsetmacro{\auxy}{2*sqrt(3)/7}

% Square variables

% Heptagon variables

% Hexagon variables



% Colors
\definecolor{lred}{HTML}{FFADAD}
\definecolor{lorange}{HTML}{FFD6A5}
\definecolor{lyellow}{HTML}{FDFFB6}
\definecolor{lgreen}{HTML}{CAFFBF}
\definecolor{lturquoise}{HTML}{9BF6FF}
\definecolor{lblue}{HTML}{A0C4FF}
\definecolor{lpurple}{HTML}{BDB2FF}
\definecolor{lpink}{HTML}{FFC6FF}


